Opportunistic Transmission of Distributed Learning Models in Mobile UAVs

In this paper, we propose an opportunistic scheme for the transmission of model updates from Federated Learning (FL) clients to the server, where clients are wireless mobile users. This proposal aims to opportunistically take advantage of the proximity of users to the base station or the general condition of the wireless transmission channel, rather than traditional synchronous transmission. In this scheme, during the training, intermediate model parameters are uploaded to the server, opportunistically and based on the wireless channel condition. Then, the proactively-transmitted model updates are used for the global aggregation if the final local model updates are delayed. We apply this novel model transmission scheme to one of our previous work, which is a hybrid split and federated learning (HSFL) framework for UAVs. Simulation results confirm the superiority of using proactive transmission over the conventional asynchronous aggregation scheme for the staled model by obtaining higher accuracy and more stable training performance. Test accuracy increases by up to 13.47% with just one round of extra transmission.

==> figure.tex <==
% \hfill
    \begin{subfigure}[b]{0.245\textwidth}
         \centering
         \includegraphics[width=130, height=110]{Figs/Simulation Results/Fig2.pdf}
         %\includegraphics[width=\textwidth, height=105]{Figs/Simulation Results/Fig2_2.pdf}
         \caption{Accuracy$\&$Overhead}
         \label{fig:Fig2}
     \end{subfigure}
   %  \hfill
  \begin{subfigure}[b]{0.245\textwidth}
         \centering
        % \includegraphics[width=\textwidth,height=105]{Figs/Simulation Results/Fig3.pdf}
         \includegraphics[width=130,height=110]{Figs/Simulation Results/Fig3.pdf}
         \caption{Accuracy $\&$ Latency}
         \label{fig:Fig3}
     \end{subfigure}
    %  \hfill
      \begin{subfigure}[b]{0.245\textwidth}
         \centering
         \includegraphics[width=130,height=110]{Figs/Simulation Results/Fig4.pdf}
         \caption{Test loss}
         \label{fig:Fig4}
     \end{subfigure}
